Random Forest Regression for continuous affect using Facial Action Units

In this paper we describe our approach to the arousal and valence track of the 3rd Workshop and Competition on Affective Behavior Analysis in-the-wild (ABAW). We extracted facial features using OpenFace and used them to train a multiple output random forest regressor. Our approach performed comparable to the baseline approach.

==> Chapters/related.tex <==
\section{Related Works}
\label{sec:related}

